MGG: Accelerating Graph Neural Networks with Fine-grained intra-kernel Communication-Computation Pipelining on Multi-GPU Platforms

The increasing size of input graphs for graph neural networks (GNNs) highlights the demand for using multi-GPU platforms. However, existing multi-GPU GNN systems optimize the computation and communication individually based on the conventional practice of scaling dense DNNs. For irregularly sparse and fine-grained GNN workloads, such solutions miss the opportunity to jointly schedule/optimize the computation and communication operations for high-performance delivery. To this end, we propose MGG, a novel system design to accelerate full-graph GNNs on multi-GPU platforms. The core of MGG is its novel dynamic software pipeline to facilitate fine-grained computation-communication overlapping within a GPU kernel. Specifically, MGG introduces GNN-tailored pipeline construction and GPU-aware pipeline mapping to facilitate workload balancing and operation overlapping. MGG also incorporates an intelligent runtime design with analytical modeling and optimization heuristics to dynamically improve the execution performance. Extensive evaluation reveals that MGG outperforms state-of-the-art full-graph GNN systems across various settings: on average 4.41X, 4.81X, and 10.83X faster than DGL, MGG-UVM, and ROC, respectively.

==> 03_related_work.tex <==
%-------------------------------------------------------------------------------
\section{Related Work and Discussion} 
\label{sect: Related Works}
%-------------------------------------------------------------------------------
%  In this section, we will given more discussion of Single-GPU and Multi-GPU GNNs.
% \subsection{GNN Basics}
% \label{sect: Graph Neural Networks}
% % \vspace{-5pt}
% Figure~\ref{fig: GNN Computation Flow} visualizes the computation flow of GNNs in one iteration. 
% GNNs compute the node feature vector (embedding) for node $v$ at layer $k+1$ based on the embedding information at layer $k$ ($k \geq 0$), as shown in Equation~\ref{eq: GNN},
% \begin{gather} \small 
% \label{eq: GNN}
%  \begin{aligned} 
%   a_{v}^{(k+1)}  &= \mathbf{Aggregate}^{(k+1)}({h_{u}^{(k)}|u\in \mathbf{N}(v)\cup h_v^{(k)}}) \\
%   h_{v}^{(k+1)}  &= \mathbf{Update}^{(k+1)}(a_{v}^{(k+1)})
% \end{aligned}   
% \vspace{-10pt}
% \end{gather}
% where $h_{v}^{(k)}$ is the embedding vector for node $v$ at layer $k$; $h_v^{(0)}$ is computed from the task-specific features of a vertex (\textit{e.g.}, the text associated with the vertex, or some scalar properties of the entity that the vertex represents) via some initial embedding mapping that is used only for this ingest of symbolic values into the embedding space; $a_{v}^{(k+1)}$ is the aggregation results through collecting neighbors' embeddings; $\mathbf{N}(v)$ is the neighbor set of node $v$.
% The aggregation method and the order of aggregation and update could vary across different GNNs. 
% Some methods~\cite{GCNConv, SageConv} just rely on the neighboring nodes while others~\cite{GATConv} also 
% leverage edge properties. 
% % by combining the dot product of the end-point nodes of each edge, along with any edge features (edge type and other attributes).
% \begin{figure} [t] \small
%     \centering
%     \includegraphics[width=0.8\columnwidth]{imgs/gnn_background.pdf}
%     % \vspace{-10pt}
%     \caption{GNN General Computation Flow.}
%     \label{fig: GNN Computation Flow}
%     % \vspace{-5pt}
% \end{figure}
% The update function is generally composed of standard NN operations, such as a single fully-connected layer in the form of $w\cdot a_{v}^{(k+1)} + b$, where $w$ and $b$ are the trainable weight and bias parameters, respectively.
% The common choices for node embedding dimensions are 16, 64, and 128, and the embedding dimension may change across different layers. After passing through several iterations of aggregation and update (\textit{i.e.}, several GNN layers), we will get the output feature embedding of each node, which can usually be used for various downstream tasks, such as node classification~\cite{kaspar2010graph, gibert2012graph, duran2017learning} and link prediction~\cite{chen2005link, kunegis2009learning, tylenda2009towards}.

\iffalse
\subsection{Single-GPU GNNs}
\label{sect: single-GPU GNNs}
With the prosperity of the GNN algorithms~\cite{GCNConv, GINConv, GATConv, SageConv}, the first wave of GNN system research focus %tony: focuses
on building and optimizing on the setting of single-GPU. One key character of these types of research is to extend the existing deep learning frameworks for traditional NNs to support GNNs~\cite{pyG,wang2019dgl}. 
% They mainly focus on programmability and generality for different GNN models but lack efficient backend support to achieve high performance.
Pytorch-Geometric (PyG)~\cite{pyG} uses a CUDA-based torch-scatter~\cite{torch-scatter} library for sparse graph operations.
% The torch-scatter design scales poorly when encountering large sparse graphs with high-dimensional node embedding. because its kernel design essentially borrows the design principles of graph-processing systems by using excessive high-overhead atomic operations to support node embedding propagation. 
Deep Graph Library (DGL)~\cite{wang2019dgl} incorporates an off-the-shelf Sparse-Matrix Multiplication (SpMM) (\textit{e.g.}, cuSPARSE~\cite{cusparse}) for simple sum-reduced aggregation~\cite{GCNConv,SageConv} and leverages its own CUDA kernel for more complex aggregation scheme with edge attributes~\cite{GINConv,GATConv}. 
Besides, efforts from runtime system~\cite{GNNAdvisor} and high-performance computing~\cite{ge-spmm, gapinGNN} community also contribute to GNN acceleration on a single GPU device. 
For instance, work from~\cite{GNNAdvisor} optimizes the GNN computation on the single GPU settings with input adaptivity by exploring the specialty of the GNN workloads, and the GPU kernel computation and memory access pattern. 
% Work from~\cite{ge-spmm} employs the coalesced row caching and coarse-grained warp merging to improve the memory and computation performance of GNN computation collaboratively. 
The key challenge of single GPU GNN computation is the insufficient device memory to accommodate the large real-world graphs, limiting their %tony: their? GNN's
applicability on wide-range of problem settings.

% \vspace{-10pt}
\subsection{Multi-GPU GNNs} 
\fi
With the increasing demands for handling large input graphs and high node embedding dimensionality, deploying the %tony:no "the"?
GNNs towards multiple GPUs raises the attention of the %tony: no "the"?
system researchers and engineers. 
Existing multi-GPU platforms~\cite{dgx-a100, tesla-v100} feature sufficient accumulated device memory and high-bandwidth connections (\textit{e.g.}, the latest NVIDIA DGX-A100~\cite{dgx-a100} comes with accumulated 8$\times$40GB device memory and offers up to 600GB/s inter-GPU transfer speed).
%
This trend results in an array of GNN computing frameworks/systems tailored for large graphs~\cite{ma2019neugraph, sysMLROC, cai2021dgcl, lin2020pagraph}. 
%
% \textcolor{blue}{Multiple GPUs based computing platforms (\textit{e.g.}, NVIDIA DGX-A100~\cite{dgx-a100} with sufficient device memory (8$\times$40GB) and high-bandwidth (up to 600GB/s) GPU inter-connections via NVLink and NVSwitch) become increasingly popular in the conventional deep-learning (\textit{e.g.}, CNN, LSTM) system, known for their high computing throughput and low-overhead performance scaling.} 
\iffalse
\begin{table}[t] \small
\centering
\caption{Local and Remote access in Multi-GPU GNNs.}
\vspace{-5pt}
\scalebox{0.78}{
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline 
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{2GPU}} & \multicolumn{2}{c|}{\textbf{3GPU}} & \multicolumn{2}{c|}{\textbf{4GPU}} \\ \cline{2-7} 
 & \textbf{Local} & \textbf{Remote} & \textbf{Local} & \textbf{Remote} & \textbf{Local} & \textbf{Remote} \\ \hline
Reddit & 50.02\% & 49.98\% & 33.67\% & 66.33\% & 25.49\% & 74.51\% \\ \hline
enwiki-2013 & 70.87\% & 29.13\% & 64.51\% & 35.49\% & 60.12\% & 39.88\% \\ \hline
ogbn-products & 53.08\% & 46.92\% & 55.67\% & 44.33\% & 33.63\% & 66.37\% \\ \hline
\end{tabular}}
\label{tbl: Local and Remote neighbor access in Multi-GPU GNNs.}
\end{table}
As we can see from Table~\ref{tbl: Local and Remote neighbor access in Multi-GPU GNNs.}, with the increase of the number of GPUs, there is an increase of the ratio for the remote access for the node embeddings, since more likely the neighbors are distributed among different GPU devices. While using more GPUs improves the computation parallelism, accessing those neighbors requires lots of irregular fine-grained remote memory access, which are essentially inefficient and high-overhead. Therefore, how to amortize the high costs of inter-GPU data communication is vital for the overall GNN execution performance on multi-GPU platforms.
\fi
NeuGraph~\cite{ma2019neugraph} introduces a novel graph shard-based graph partitioning and inter-GPU partition forward strategy to handle large graphs. 
% that cannot be processed by using only one GPU. 
ROC~\cite{sysMLROC} proposes a learning-based graph partitioning strategy to reduce the unnecessary CPU-to-GPU data communication. 
% Note that both \textit{NeuGraph and ROC are host-memory-based designs, where all node embeddings are maintained at the large host memory. And a subset of node embeddings will be transferred from host to device before the aggregation.}
DGCL~\cite{cai2021dgcl} develops an optimized distributed graph communication library for efficient GNN training on multiple GPUs. 
$P^{3}$~\cite{P3} uses large graph mini-batching and a pipeline push-pull parallelism for distributed GNN training. 
\fix{However, none of them has spot the potential of overlapping the data communication and the kernel computation to improve GNN performance.}

% \fix{In this work, we provide the first comprehensive exploration of SHMEM in handling GNN computation, And we demonstrate the significance of balancing workload at different levels of granularity and the benefits of overlapping the computation and communication in a fine-grained way. Future applications that can potentially benefit from SHMEM would come with \textit{fine-grained communication during the computation}. The key to make the most of SHMEM is to \textit{carefully matching the communication workload and appropriate size of computation workload.} This would motivate us to try 1) various \textit{workload-partition} techniques on either the communication or computation workload, and 2) diverse \textit{workload-overlapping} strategies, so that we can largely hide the communication latency while maximizing hardware performance.}
%
% \iffalse
% However, these existing multi-GPU solutions could find several shortcomings: 
% 1) graph mini-batching via neighbor sampling could hurt the GNN model accuracy;
% 2) the decoupled communication and computation resulting in communication bottleneck, and
% 3) hard-coded design with limited tuning flexibility. 
% Our \Mname~effectively address all these problems via a novel SHMEM-based multi-GPU system design and optimization strategies for original GNN algorithms.
% \fi
%
% In contrast, our \Mname~design can balance the workload and overlap the computation and communication with NVSHMEM~\cite{nvshmem} technique; 
% 2) balance workload and reduce computation irregularity through efficient hierarchical workload management; 3) adapt towards different input settings by tunable design parameters.

\iffalse
\subsection{NVSHMEM} 
{NVSHMEM~\cite{nvshmem} is a new type of inter-GPU communication programming library that implements OpenSHMEM~\cite{openSHMEM} for NVIDIA GPU clusters. 
%
It provides a ``shared'' global memory space across
multiple GPUs that allow for fine-grained inter-GPU data movement and synchronization directly inside a CUDA kernel. 
%
% NVSHMEM is created to address an issue in programming
% GPU-based extreme-scale systems such as Summit. Currently,
Existing design for multi-GPU DNN computation is to use NCCL+CUDA libraries (cuDNN~\cite{cuDNN}, cuBLAS~\cite{cublas}) for programming.
The whole multi-GPU application consists of a separate communication and computation phase, where CPUs coordinate the execution on the GPUs and exchange data using NCCL while GPUs handle the workloads that are offloaded by CPUs.
This CPU-GPU collaboration model incurs performance overheads caused by communication-computation transition and limits the scalability of HPC applications.}

{Using NVSHMEM, the communication and computation can be fused into one GPU kernel to minimize synchronization with the CPU.
%
Meanwhile, GPU and network utilization would also be largely improved since the additional overheads, such as launching many small kernels, will largely be reduced.
%
NVSHMEM can also effectively hide the communication latency by interleaving the computation and communication. GPU SMs warp-level scheduler can serve other active warps when the current warp is busying in communication through NVSHMEM.
% but owing to single-cycle warp scheduling on the GPU, the latency can be hidden not only to local GPU device memory but also to remote GPU memory over a network.
%
Besides, NVSHMEM can ease the programming efforts. The ``shared'' global memory provides an easy way for one GPU kernel to access the data at another GPU by simply using the targeted GPU ID and the offset of the ``shared'' global memory address on that GPU. Moreover, the communication primitives of NVSHMEM are one-sided, such as PUT and GET. There is no need for more complicated designs for carefully handling communication hanging/deadlocking when using Send-Receive semantics in NCCL.} 
% Besides SPMD-style programming and incremental improvements, a programmer will not have to rely on a hybrid model to orchestrate and overlap between different phases of
% the application. Restructuring the application code to overlap
% independent compute and communication phases makes the
% application code complex. The benefit of such restructuring
% diminishes when the problem size per GPU becomes smaller
%
The existing application of NVSHMEM covers traditional deep-learning (\textit{e.g.}, Livermore Big Artificial Neural Network~\cite{LBANN}) and scientific computing (\textit{e.g.}, quantum chromodynamics~\cite{wilczek2000qcd}) applications, which are more regular in remote memory access with relatively smaller communication and computation ratio. In this paper, we are exploring the benefits of NVSHMEM in an all new GNN domain with highly irregular computation with more intensive communication during the aggregation. 
\fi

==> 05_algorithm_design.tex <==
\section{Multi-GPU GNN Algorithm Design}
\label{sect: Multi-GPU GNN Algorithm Design}
In this section, we will discuss about our MGG algorithmic design. As illustrated in Algorithm~\ref{algo: Neighbor Aggregation on Translated Graph.}, MGG sparse computation can be divided in to several major steps. Initially, we load the graph data from the disk through graph loader, and we will then put the graph structure in CSR and graph node embeddings into the host memory. Note that this step is collaboratively handled by all working threads of the whole system. Then we will start our multi-GPU execution region, which will be executed by each worker thread and its corresponding GPU. The corresponding execution model is shown in Figure~\ref{}. \todo{add a overall Figure here}. For each worker thread on CPU, it will fetch a slice of input graph graph structural. \todo{here we also tacle the workload imbalance problem via edge-balanced targeted-node partitioning. adding the NN part description and the gradient and backward propagation routine.}
Then it will split the slice according to the neighbor aggregation workload depending on whether fetching such neighbor requires local/remote access. 
Once this step is done, we will apply neighbor partitioning on each type of workload lists, then launch our MGG kernel running on each GPU to process such workload.
Once all GPU kernels return, we will basically copy the result from each GPU device memory to a continuous memory on host memory to achieve final result concatenation. 
\begin{algorithm}[t] \small
  \caption{Multi-GPU Sparse GNN Operation.}
  \label{algo: Neighbor Aggregation on Translated Graph.}
\SetAlgoLined
  \SetKwInOut{Input}{input}
  \SetKwInOut{Output}{output}
  \Input{Graph dataset path ($\mathit{gPATH}$) and \# GPUs ($nGPU$).}
  \Output{Updated node embedding matrix ($\mathbf{\hat{X}}$).}
  \tcc{Load graph data to host memory.}
  $\mathit{rowPtr}$, $\mathit{colIdx}$, $\mathbf{X}$ = \textbf{GLoader}($\mathit{gPATH}$) \;
  \tcc{\textcolor{red}{--*--BEGIN: Multi-GPU Execution Region.--*--}}
  \tcc{Step-1: Target-based Distribution (TBD).}
  $\mathit{rptr\_sli}$, $\mathit{cidx\_sli}$ = \textbf{TBD}($\mathit{rowPtr}$, $\mathit{colIdx}$, $\mathit{GPUIdx}$)\;
  
  \tcc{Step-2: Local-remote split (LRS).}
  $\mathit{lc\_info}$, $\mathit{re\_info}$ = \textbf{LRS}($\mathit{rptr\_sli}$, $\mathit{cidx\_sli}$)\;

  \tcc{Step-3: Neighbor-based Partitioning.}
  $\mathit{p\_lc}$ = \textbf{BuildPartition}($\mathit{lc\_info}$)\;
  $\mathit{p\_re}$ = \textbf{BuildPartition}($\mathit{re\_info}$)\;
   
  $\mathbf{\hat{X}\_sli}$ = \textbf{MGG\_Kernel}($\mathit{p\_lc}$, $\mathit{p\_re}$, $\mathit{X\_sli}$)\;
   
  \tcc{\textcolor{red}{--*--END: Multi-GPU Execution Region.--*--}}
 
 \tcc{Concatenate all embedding slices on host.}
 $\mathbf{\hat{X}}$ = \textbf{Concat}($[\mathit{X\_sli_1}, ..., \mathit{X\_sli_{nGPU}}]$);
\end{algorithm}

==> 07_related_work.tex <==
\section{Related Work}




% \section{Range-constrained Binary Search.}
% Please see Algorithm~\ref{algo: Range-constrained Binary Search.}.
% \label{appendix: Range-constrained Binary Search.}
% \begin{algorithm}[h] \small
%   \caption{Range-constrained Binary Search.}
%   \label{algo: Range-constrained Binary Search.}
% \SetAlgoLined
%   \SetKwInOut{Input}{input}
%   \SetKwInOut{Output}{output}
% %   \DontPrintSemicolon
%   \SetKwFunction{FMain}{binSearch}
%   \SetKwProg{Fn}{Function}{:}{}

%   \Input{Graph node pointer array ($\mathit{nPtr}$), edge list array ($\mathit{eList}$) , and the number of GPUs ($\mathit{numGPUs}$).}
%   \Output{list of graph edge split points ($\mathit{numGPUs} - 1$).}
%     $\mathit{outList} = []$; $\mathit{lastPos} = 0$\;
%     \tcc{Compute approximated \#edges per GPU.}
%     $\mathit{ePerGPU}$ = $(len(eList) + \mathit{numGPUs} - 1)/\mathit{numGPUs}$\;
%     \For{$sId$ \textbf{in} [0, ..., $\mathit{numGPUs} - 1$]}{
%         $nid$ = $\mathit{\texttt{binSearch}}(\mathit{nPtr}, \mathit{ePerGPU}, \mathit{lastPos}, \mathit{numNodes})$\;
%         $\mathit{lastPos} = nid$\;
%         $\mathit{outList}.\mathit{append}(nid)$\;
%     }
%     \textbf{return} $outList$\;
% \BlankLine
% \tcc{Search split points on $nPtr$.}
% \Fn{\FMain{$nPtr$, $ePerGPU$, $lastPos$,                      $numNodes$}}{
%       $i = lastPos$; $j = numNodes$\;
%       $target = \min(nPtr[i] + ePerGPU, nPtr[numNodes])$\;
%         \While{$i < j$}{
%         $mid = (nPtr[i] + nPtr[j])/2$\;
%         \uIf{$mid > target$}{    
%             $j = (i + j) / 2$\;
%         }
%         \uElse{
%             $i = (i + j) / 2$\;
%         }
%         }
%     \KwRet i\;
%  }
% \end{algorithm}
% \section{GPU SM Shared Memory Design}
% \label{appendix: GPU SM Shared Memory Design}
% Please see Listing~\ref{code: shared memory design.}.
% \begin{figure}[t] \small
% % \vspace{-10pt}
% \begin{lstlisting}[caption=GPU SM Shared Memory Design.,label={code: shared memory design.}, style=tt3]
% // GPU Kernel with Computation and Communication 
% __global__ MGG_kernel (param1, param2, ...){
%     // Get the global thread ID.
%     int tid =  blockIdx.x * blockDim.x + threadIdx.x;  
%     // Get the global warp ID.
%     int warpId = tid / WARP_SIZE; 
%     // Get the block-level warp ID.
%     int block_warpId = threadIdx.x / WARP_SIZE;
%     // Get the warp-level thread ID (laneid).
%     int laneid = threadIdx.x % WARP_SIZE;   
%     // Define the dynamic shared memory.
%     extern __shared__ int part_meta[];          
%     // Starting address for node neighbors IDs.
%     int *partial_ids = part_meta;
%     // Starting address for partial aggregation result.
%     float *partial_results = (float*)&part_meta[partSize*warpPerBlock];
%     // Starting address for remotely-fetched embeddings.
%     float *tmp_local = (float*)&partial_results[partSize*warpPerBlock*dim];   
%     // Calculate the offset for each warp.
%     int ids_offset = warpId*partSize;
%     int partial_offset = warpId*partSize*dim;
%     int tmp_offset = warpId*partSize*dim;
%     // Warp-level NVSHMEM for remote neighbor fetching...
%     // Warp-level aggregation computation ...
% }
% // ----------launching the kernel on CPU HOST-------------
% MGG_host (param1, param2, ...){
%     // Calculate the GPU parameters.
%     int n_parts = max(lc_parts, re_parts);
%     int block = warpPerBlock * WARP_SIZE;
%     int grid = (n_parts * WARP_SIZE + block  - 1) / block; 
%     int shared_memory_size = partSize*warpPerBlock*sizeof(int) + 2*partSize*warpPerBlock*dim*sizeof(float); 
%     // Launch the GPU kernel.
%     MGG_kernel <<<grid, block, shared_memory_size>>> (param1, param2, ...);
%     // Other following operations ...
% }
% \end{lstlisting}
% % \vspace{-5pt}
% \end{figure}


% \section{Additional Discussion} 
% \label{appendix: discussion}
% \textbf{Graph Partitioning: }
% Our NVSHMEM-based designs/optimizations could also support other graph partitioning strategies from prior graph processing and GNN work. There are several major categories.
% %
% \textbf{\textit{1) Locality-driven partitioning}} (e.g., Rabbit order~\cite{rabbit-order}) minimizes the communication/synchronization cost in distributed graph processing/GNN computing. \Mname~can effectively accommodate such reduced-communication cases through dynamic kernel re-configuration (e.g., finetuning the interleaving distance and warp-to-block mapping) to maximize the communication and computation efficiency.
% %
% \textbf{\textit{2) Workload-driven partitioning}} (e.g., NeuGraph~\cite{ma2019neugraph}) balances the irregular graph/GNN workload among different devices. Our current design be easily adapted to handle such cases by inserting device synchronization primitives (NVSHMEM collective communication primitives, such as \texttt{nvshmem\_float\_sum\_reduce}) for maintaining data consistency among different replicas.
% % \begin{table}[h] \small
% % \centering
% % \vspace{-5pt}
% % \caption{DLRM with \Mname~support in Embedding Table Lookup.}
% % \vspace{-5pt}
% % \begin{tabular}{l|r | r }
% % \specialrule{.1em}{.05em}{.05em}
% % \textbf{Implementation} & DLRM~\cite{naumov2019deep} & DLRM (\Mname)  \\
% % \hline\hline
% % \textbf{Time (ms)} & 315.27 & 119.66  \\
% % \specialrule{.1em}{.05em}{.05em}
% % \end{tabular}
% % \label{tbl: pipeline on DLRM}
% % % \vspace{5pt}
% % \end{table}

% \iffalse
% \textbf{Design Generality: }
% {\Mname~can be generalized to other similar applications.
% %
% One typical example is the popular deep-learning recommendation model (DLRM)~\cite{naumov2019deep, zhang2019deep, gupta2020architectural}, which is mainly throttled by the performance of its sparse embedding table lookup. 
% In multi-GPU DLRM, the large embedding tables are partitioned by rows/columns and stored in different GPUs. The DLRM inputs (embedding access queries) will request to fetch embeddings from other tables on different GPUs. We improve the mainstream DLRM system~\cite{naumov2019deep} with \Mname~to accelerate embedding lookup and compare with the original system (with NCCL)~\cite{naumov2019deep} under 4-GPU settings on Criteo Kaggle~\cite{kaggle} dataset. Table~\ref{tbl: pipeline on DLRM} shows that DLRM with \Mname~effectively reduces the time of look up (2.64$\times$). Since the fine-grained remote memory access of \Mname~can remove redundant inter-GPU traffic induced by NCCL, which can only handle dense \& regular communication paradigm.
% % Our pipelined design could be used to overlap embedding collecting and the embedding interaction with associative operators (e.g., sum/min/max reduction) to reduce the overall computing latency and improve system utilization.
% % However, for embedding iterations with non-associative operators (e.g., concatenation with orders), such computation-communication overlapping design would be less effective due to the necessary synchronization to guarantee the output correctness.
% }
% \textbf{Hardware Generality: } 
% Our design can also be adapted toward other hardware platforms with similar communication support. 
% For instance, on the multi-CPU based platform with OpenSHMEM~\cite{openSHMEM}, our current GPU kernel design can be rewritten as regular C++ functions mixed with OpenSHMEM primitives (in place of NVSHMEM primitives) to be executed on CPU-based distributed platforms. On the CPU, since there is no notion of thread warp/block, the program mainly relies on thread/process-level parallelism. Thus, we need to determine the runtime configurations (e.g., the total number of CPU threads) so that we can balance the computation parallelism and the computation-communication pipelining efficiency. We need to do additional profiling to get the relative latency cost of computation and communication on multi-CPU platforms and adjust the way/pattern of overlapping the computation and communication (e.g., the interleaving distance). 
% \fi

% \iffalse
% \section{Discussion}
% Prior $\S$\ref{sect: Background and Motivation} overviews the existing multi-GPU GNN systems. This section will discuss the techniques for scaling multi-GPU deep learning and its applicability in GNNs.

% % \textbf{Collective Communication (CC)}~\cite{nccl, sergeev2018horovod,rccl} is a common strategy for scaling dense DNN training. 
% % Collective operations exhibit a regular coarse-grained communication paradigm with the same set of operations (e.g., AlltoAll and AllReduce) for data exchange.
% % %
% % Among existing CC designs, NCCL~\cite{nccl} delivers state-of-the-art communication performance on NVIDIA GPUs. 
% % %
% % However, NCCL could hardly demonstrate its advantages in GNNs.
% % %
% % First, NCCL is designed for regular communication patterns, while communication in sparse GNN computation is highly irregular.
% % Second, NCCL has to interrupt the current GPU kernel for communication, leading to non-trivial costs for CPU-GPU context switching.

% \textbf{Unified Virtual Memory (UVM)}~\cite{unifiedMemory} maintains a global ``virtual'' view of a single address space spanning across CPU and GPU memory. 
% With UVM, multi-GPU programming can be simplified as single-GPU programming, where the data physical location is transparent~\cite{unifiedMemory, yu2019hierarchical,kim2020batch} to programmers.
% %
% In UVM, whenever a GPU kernel wants to access the data that is currently absent from GPU memory, a GPU-side page fault will happen and a CPU-to-GPU page migration will be triggered to fetch the corresponding data from the host memory to GPU memory on demand. However, the data access in UVM is coarse-grained (4KB per memory page) and its access speed bounded by the PCIe connection.

% % However, applying UVM in GNNs are facing several challenges:
% % First, GNN computation relies on highly irregular memory access. using UVM would trigger lots of GPU-side page-fault for frequently fetching remote data. And the coarse-grained memory pages migration is costly.
% % %
% % Second, UVM can only count on PCIe connection for CPU-to-GPU data transferring and would stall the massively parallel and high-performance GPU execution.

% \textbf{Zero-Copy Memory} (ZC)~\cite{zero-copy} enables GPU threads to directly access host memory without the engagement of CPUs. 
% ZC allocates memory that is physically pinned in CPU host memory and shares the data pointer of pinned host memory to the GPU kernel. 
% The GPU kernel-originated data transfers of ZC can automatically overlap kernel execution. 
% Different from UVM (KB-level access granularity), communication using ZC is more fine-grained (hundreds of bytes) and the access pattern of ZC also depends on the GPU kernel design. 
% However, the memory access cost and efficiency of ZC would vary depending on the memory address location, memory access pattern, and access granularity.
% ZC is also the key technique used by Pytorch-Direct~\cite{PyTorch-Direct}, which is the major communication backend of DGL~\cite{wang2019dgl} for large GNN input.

% \textbf{SHMEM}~\cite{openSHMEM, nvshmem,rocsheme} is a typical multi-device parallel programming model. In SHMEM, a global memory address space is logically constructed based on the memory subspace of individual workers (\textit{e.g.}, CPU/GPU). 
% Among existing SHMEM designs, NVHSMEM~\cite{nvshmem} is designed for inter-GPU communication on NVIDIA GPUs. The highlight of NVSHMEM is its GPU-initiated fine-grained data movement across GPUs.
% %
% Compared with ZC, NVSHMEM-based communication does not require allocating the pinned memory space on the CPU host and the communication happens only among GPUs without CPU engagement.
% %
% The existing application of NVSHMEM focuses on conventional DNNs~\cite{LBANN}, which are \textit{regular} in remote data access. \Mname~explores the benefits of NVSHMEM in an all-new GNN domain with \textit{irregularly sparse} computation and communication. 
% \fi
